Interplay between Network Topology and Dynamics in Neural Systems

This thesis is a compendium of research which brings together ideas from the fields of Complex Networks and Computational Neuroscience to address two questions regarding neural systems: 1) How the activity of neurons, via synaptic changes, can shape the topology of the network they form part of, and 2) How the resulting network structure, in its turn, might condition aspects of brain behaviour. Although the emphasis is on neural networks, several theoretical findings which are relevant for complex networks in general are presented -- such as a method for studying network evolution as a stochastic process, or a theory that allows for ensembles of correlated networks, and sets of dynamical elements thereon, to be treated mathematically and computationally in a model-independent manner. Some of the results are used to explain experimental data -- certain properties of brain tissue, the spontaneous emergence of correlations in all kinds of networks... -- and predictions regarding statistical aspects of the central nervous system are made. The mechanism of Cluster Reverberation is proposed to account for the near-instant storage of novel information the brain is capable of.

==> ant/ant.tex <==
%\documentclass[a4paper,10pt]{article}
%\usepackage{graphicx}
%\usepackage{amssymb}

\chapter{Preamble:\\The ant, the grasshopper and complexity} % Write in your own chapter title
%\section{Preamble: The ant, the grasshopper and complexity}
%\label{Chapter4}
\lhead{\emph{Preamble: The ant, the grasshopper and complexity}} % Write in your own chapter title to set the page header

Once upon a time, in a charming and peaceful little valley, a grasshopper sat under the shade
of a sunflower, idly strumming up a tune, when a young worker ant came into view. The
grasshopper watched as she trundled her way laboriously up an incline under the weight of a
large piece of leaf. When she was close enough, he hailed her:
\\
`Ahoy there, friend. I hope I won't seem tactless if I point out what a singularly cumbersome
bit of leaf you have there. Would you not rather put it down for a while and join me for a
quick jam session? You could bang along on some twigs or something.'
\\
`Thank you for the offer, but I must continue on my way,' replied the ant, glancing up in
slight surprise at being thus addressed.
\\
`Oh, what a pity,' the grasshopper rejoined. `And where, if I may be so bold as to inquire,
would you be taking your rather unappetising ration of cellulose?'
\\
`Well, I can't say I really know... I just follow this trail of pheromones I've come across. I'm sure
it's for some noble purpose though.'
\\
`Ah, that must be reassuring. And I suppose when you get to wherever it is you don't know
you're going you intend to eat your bit of leaf...'
\\
`Oh no, I can't digest something like this -- who do you take me for?'
\\
`You can't? Well, how strange...'
\\
`What's strange?'
\\
`However did an animal evolve which, instead of engaging in biologically reasonable (not to
mention enjoyable) activities, such as playing music to attract sexual partners, prefers to lug
useless bits of leaf about? How on earth can that serve to spread your genes?'
\\
`I'm not interested in music or sex, whatever those are. I just follow simple rules, like all my identical
sisters. You could say we're automata.'
\\
`Thanks, I was going to but wasn't sure whether you'd be offended. Well, let me wish you an
agreeable day of toil, you frigid little automaton.'
\\

With that, the grasshopper gave a big leap into the air, slightly exasperated by the folly so
often displayed by his fellow insects. Looking down, he spotted a few more ants, all carrying
leaves in the same direction as the one he had just met. Intrigued, he fluttered slightly higher
(since grasshoppers can, actually, fly, if not all that well). He realised the ants were all heading
for a nest some way off. In fact, there were many ant trails leading to various sources of food.
It dawned on the grasshopper that although the individual ants were just boring little morons
idiotically following rules, the nest as a whole was managing to find the closest leaves, bring
them back along optimal routes, and feed them to its plantations of fungi. The colony was
behaving like an intelligent organism, in some respects not so different from he himself, who
functioned thanks to the cells of his body -- each with the same genome, like the ants --
cooperating through the obedience to relatively simple rules.
\\

This thought impressed the grasshopper very much, driving him to flutter even higher so as to
see things in greater perspective. From there he considered the apparently fragile web of
trophic, parasitical and symbiotic interactions linking all the living beings in the valley -- a
network which nonetheless must have evolved a particularly robust structure not to shatter at
the first environmental fluctuation. He became so enthralled by the idea of such complexity on
one scale emerging from simplicity on another that he didn't even pay any attention to an
attractive young grasshopperess making her wanton way just below him. Instead, he couldn't
help fearing that a butterfly he noticed gently flapping his wings would probably set off a
hurricane somewhere. As he flew ever higher, he began to see snowflakes glide by,
overwhelmingly intricate and beautiful patterns self-organised out of the simplest little water
molecules. Finally he was so high that he began to reflect on how the very stellar systems,
galaxies,
%cumuli and super-cumuli of galaxies
clusters, superclusters, filaments of galaxies...
-- of which his whole world was but an
infinitesimal component -- also interacted with each other via the simple rules of gravity and
pressure to form objects marvellous beyond conception.
\\

What he didn't notice until it was too
late, as he left behind the cosy protection of the atmosphere, was how ultraviolet sunlight and
ionising cosmic rays were steadily burning his wings each to a crisp. Beginning to fall, he only
hoped he would have time to consider the several morals to his tragic tale.
\\

After a while spent plummeting to his doom he realised that, the freefall terminal velocity and life expectancy of a grasshopper being what they respectively were, he would most likely die peacefully of old age somewhere along his way down -- never again contemplating his Edenic valley except, like some prophetic locust, from afar.


==> prl/ideas.tex <==
\chapter{More possible appendices and things}
\label{AppendixB}
\lhead{Appendix B. \emph{More possible appendices ad things}}}

\begin{itemize}
 \item 
Stochastic processes

\item
Emergence of scaling in nature

\item
Constructing networks: hidden variables etc. (though perhaps it would be better to discuss this in the introduction)

\item
Other (more realistic) neural models 

\item
Summery of thesis in Spanish

\end{itemize}



==> prl/prl_old.tex <==
%\documentclass
%[twocolumn,showpacs,preprintnumbers,prl,tightenlines,
%superscriptaddress,footinbib]{revtex4}%
%\usepackage{amssymb}
%\usepackage{graphicx}
%\usepackage{dcolumn}
%\usepackage{bm}
%\usepackage{amsmath}
%\usepackage{amsfonts}%
%\setcounter{MaxMatrixCols}{30}
%\providecommand{\U}[1]{\protect\rule{.1in}{.1in}}
%\providecommand{\U}[1]{\protect\rule{.1in}{.1in}}
%\begin{document}

%\title{The entropic origin of disassortativity in complex networks}
%\author{Samuel Johnson\thanks{samuel@onsager.ugr.es}, Joaqu\'{\i}n J. Torres,
%  J. Marro, and Miguel A. Mu\~{n}oz \\ \small{\textit{Departamento de
%      Electromagnetismo y F\'{\i}sica de la Materia, and\\ Institute
%      \textit{Carlos I}\ for Theoretical and Computational Physics,\\ Facultad
%      de Ciencias, University of Granada, 18071 Granada, Spain.}}}

\chapter{Entropic origin of disassortativity in complex networks}
\label{Chapter_PRL}
\lhead{\emph{Entropic origin of disassortativity in complex networks}}




%\begin{abstract}
\begin{quotation}
\begin{center}
{\bf Abstract}
\end{center}
  Why are most empirical networks, with the prominent exception of
  social ones, generically degree-degree anticorrelated, i.e.
  \textit{disassortative}? With a view to answering this long-standing
  question, we define a general class of degree-degree correlated
  networks and obtain the associated Shannon entropy as a function of
  parameters. It turns out that the maximum entropy does not typically
  correspond to uncorrelated networks, but to either
  \textit{assortative} (correlated) or \textit{disassortative}
  (anticorrelated) ones. More specifically, for highly heterogeneous
  (scale-free) networks, the maximum entropy principle usually leads
  to disassortativity, providing a parsimonious explanation to the
  question above. Furthermore, by comparing the correlations measured
  in some real-world networks with those yielding maximum entropy
for the same degree sequence, 
 we find
a remarkable
agreement in various cases.
  Our approach provides a {\it neutral model} from which, in the absence
  of further knowledge regarding network evolution, one can obtain the expected value of
  correlations. In cases in which empirical observations deviate from
  the neutral predictions -- as happens in social networks -- one can then
  infer that there are specific correlating mechanisms at work.
\end{quotation}
%and estimate their nature.
%\end{abstract}

%\pacs{89.75.Fb, 89.75.Hc, 05.90.+m}

% 89.75.Fb Structures and organization in complex systems 89.75.Hc
% Networks and genealogical trees 89.70.+c Information theory and
% communication theory 05.90.+m Other topics in statistical physics,
% thermodynamics, and nonlinear dynamical systems

%\maketitle

\section{Assortativity of networks}

Complex networks, whether natural or artificial, have non-trivial topologies
which are usually studied by analysing a variety of measures, such as the degree
distribution, clustering, average paths, modularity, etc.
\cite{Albert_rev,Dorogovtsev_book,Pastor-Satorras_book,Newman_rev,Boccaletti} The mechanisms which lead to a particular
structure and their relation to functional constraints are often not clear
and constitute the subject of much debate \cite{Newman_rev, Boccaletti}. When
nodes are endowed with some additional ``property,'' a feature known as
\textit{mixing} or \textit{assortativity} can arise, whereby edges are not
placed between nodes completely at random, but depending in some way on the property in
question. If similar (dissimilar) nodes tend to wire together, the network is
said to be \textit{assortative} (\textit{disassortative})
\cite{Newman_mixing_PRL, Newman_mixing_PRE}.

An interesting situation is when the property taken into account is the degree
of each node -- i.e., the number of neighboring nodes connected to it. It
turns out that a high proportion of empirical networks -- whether biological,
technological, information-related or linguistic -- are disassortatively
arranged (high-degree nodes, or hubs, are preferentially linked to low-degree
neighbors, and viceversa) while social networks are usually assortative. Such
degree-degree correlations have
%been found to have
important consequences for
network characteristics such as connectedness and robustness
\cite{Newman_mixing_PRL, Newman_mixing_PRE}.

However, while assortativity in social networks can be explained
taking into account homophily \cite{Newman_mixing_PRL, Newman_mixing_PRE} or modularity
\cite{Newman_social}, the widespread prevalence and extent of
disassortative mixing in most other networks remains somewhat
mysterious. Maslov \textit{et al.} found that the restriction of having at most one
edge per pair of nodes induces some disassortative correlations
in heterogeneous networks \cite{Maslov},
and Park and Newman showed how this analogue of the Pauli exclusion principle leads to the edges following Fermi statistics \cite{Park_correlations} (see also \cite{Roma}).
However, this
restriction
is not sufficient to fully account for
empirical data. In general,
when one attempts to consider computationally
all the networks with the same distribution as a
given empirical one,
the mean assortativity is not necessarily zero
\cite{Zhao}. But since some ``randomization'' mechanisms induce positive correlations and others negative ones \cite{Farkas, Johnson_JSTAT}, it is not clear how the phase space can be properly sampled numerically.

In this letter, we show that there is a general reason, consistent
with empirical data, for the ``natural'' mixing of most networks to be
disassortative. Using an information-theory approach we find that the
configuration which can be expected to come about in the absence of specific additional
constraints turns out not to be, in general, uncorrelated. In fact,
for highly heterogeneous degree distributions such as those of the
ubiquitous scale-free networks, we show that the expected value of the
mixing is usually disassortative: there are simply more possible
disassortative configurations than assortative ones. This result
provides a simple topological answer to a long-standing question. Let
us caution that this does {\it not} imply that all scale-free networks
are disassortative, but only that,
in the absence of further information on the mechanisms behind their evolution, this is the neutral expectation.

\section{The entropy of network ensembles}

The topology of a network is entirely described by its adjacency
matrix $\hat{a}$; the element $\hat{a}_{ij}$ represents the number of
edges linking node $i$ to node $j$ (for undirected networks, $\hat{a}$
is symmetric). Among all the possible microscopically distinguishable
configurations a set of $L$ edges can adopt when distributed among $N$
nodes, it is often convenient to consider the set of configurations
which have certain features in common -- typically some macroscopic
magnitude, like the degree distribution. Such a set of configurations
defines an \textit{ensemble}. In a seminal series of papers Bianconi
has determined the partition functions of various ensembles of random
networks and derived their statistical-mechanics entropy
\cite{Bianconi_entropy, Bianconi_ensembles, Anand}. This allows the author to estimate the
probability that a random network with certain constraints has of
belonging to a particular ensemble, and thus assess the relative
importance of different magnitudes and help discern the mechanisms
responsible for a given real-world network. For instance,
she shows
that scale-free networks arise naturally when the total entropy
is restricted to a small finite value. Here we take a similar
approach: we
obtain the Shannon information entropy encoded in the
distribution of edges. As we shall see, both methods yield the same results
\cite{Jaynes, Anand}, but for our purposes the Shannon entropy is more tractable.

The Shannon entropy associated with a probability distribution $p_m$ is
$s=-\sum_{m}p_{m}\ln(p_{m})$, where the sum extends over all possible outcomes
$m$. For a given pair of nodes $(i,j)$, $p_{m}$ can be considered to represent
the probability of there being $m$ edges between $i$ and $j$. For simplicity,
we shall focus here on networks such that
$\hat{a}_{ij}$ can only take values $0$ or $1$,
 although the method is applicable to any number of edges allowed. 
In this case, we have only two terms: $p_{1}=\hat{\epsilon}_{ij}$ and
$p_{0}=1-\hat{\epsilon}_{ij}$, where $\hat{\epsilon}_{ij}\equiv
E(\hat{a}_{ij})$ is the expected value of the element $\hat{a}_{ij}$ given
that the network belongs to the ensemble of interest. The entropy associated
with pair $(i,j)$ is then $ s_{ij}=-\left[\hat{\epsilon}_{ij} \ln
 (\hat{\epsilon}_{ij})+(1-\hat{\epsilon}_{ij})\ln(1-\hat{\epsilon}_{ij})\right]
$, while the total entropy of the network is $S=\sum_{ij}^{N}s_{ij}$: 
\begin{equation}
 S=-\sum_{ij}^{N}\left[\hat{\epsilon}_{ij} \ln (\hat{\epsilon}_{ij})
  +(1-\hat{\epsilon}_{ij})\ln(1-\hat{\epsilon}_{ij})\right].
\label{eq_s_exact}
\end{equation}
Since we have not imposed symmetry of the adjacency matrix,
this expression is in general valid for directed networks. For
undirected networks, however, the sum is only over $i\leq j$, with the
consequent reduction in entropy.

For the sake of illustration, we shall estimate the entropy of the Internet at
the autonomous system (AS) level and compare it with the values obtained in
\cite{Bianconi_entropy, Bianconi_ensembles, Anand} assuming the network belongs to two different
ensembles: the fully random graph, or Erd\H{o}s-R\'{e}nyi (ER) ensemble, and the
\textit{configuration} ensemble with a scale-free degree distribution ($p(k)\sim k^{-\gamma}$)
\cite{Newman_rev} and structural cutoff, $k_{i}<\sqrt{\langle k\rangle N}$,
$\forall i$ \cite{Bianconi_entropy, Bianconi_ensembles, Anand} ($\langle k\rangle$ is the mean degree). In this example, we assume the network to
be sparse enough to expand the term $\ln(1-\hat{\epsilon}_{ij})$ in
Eq. (\ref{eq_s_exact}) and keep only linear terms. This reduces
Eq. (\ref{eq_s_exact}) to
$
S_{sparse}\simeq-\sum_{ij}^{N}\hat{\epsilon}_{ij}
[\ln(\hat{\epsilon}_{ij})-1]+O(\hat{\epsilon}_{ij}^{2}).
$
In the ER ensemble, each of $N$ nodes has an equal probability of receiving each of $\frac{1}{2}\langle k\rangle N$ undirected edges.
So, writing $\hat{\epsilon}_{ij}^{ER}=\langle k\rangle/N$, we have
$
S_{ER}=-\frac{1}{2}\langle k\rangle N\left[\ln\left(\langle k\rangle/N\right)-1\right].
$
The configuration ensemble, which imposes a given
degree sequence $(k_{1},... k_{N})$, is defined via the expected value of the
adjacency matrix:
$\hat{\epsilon}_{ij}^{c}=k_{i}k_{j}/(\langle k\rangle
N)$ \cite{Newman_rev,Johnson_EPL}. This value 
leads to
$ S_{c}=\langle k\rangle N[\ln(\langle k\rangle
N)+1]- 2N\langle k \ln k\rangle,
$ where $\langle \cdot \rangle \equiv N^{-1}\sum_{i}(\cdot)$ stands for
an average over nodes.
\begin{figure}
[tbh]
\begin{center}
\includegraphics
%[height=5cm, width=7.5cm]%
[scale=0.75]
{PRL/fig1_PRL.eps}
\caption{(Color online) Evolution of the Internet at the AS
  level. Empty (blue) squares and circles:
entropy per node
  of randomized networks in the fully random and in the configuration ensembles,
  as obtained by Bianconi (hence the ``B'' superscription) \cite{Bianconi_entropy, Bianconi_ensembles, Anand}. Filled
  (red) triangles and diamonds:
Shannon entropy
for an ER network and a scale-free one with $\gamma=2.3$, respectively.
}%
\label{fig_int}%
\end{center}
\end{figure}

Fig. \ref{fig_int} displays the entropy per node obtained in
\cite{Bianconi_entropy, Bianconi_ensembles, Anand} for the first two levels of approximation
(ensembles) to the Internet at the AS level, first
taking into account only the numbers of nodes $N$ and edges $L=\frac{1}{2}\langle
k\rangle N$, and then also the degree sequence. Alongside these, we
plot the 
Shannon entropy
both for an ER random network,
(which coincides exactly with Bianconi's
expression), and for a scale-free network with $\gamma=2.3$
(the slight disparity arising from this exponent's changing a little with time).


\section{Entropic origin of disassortativity}

We shall now go on to analyse the effect of degree-degree correlations on the
entropy.
In the configuration ensemble, the expected value
of the mean degree of the neighbors of a given node is $
k_{nn,i}=k_{i}^{-1}\sum_{j}\hat{\epsilon}_{ij}^{c}k_{j}=\langle
k^{2}\rangle/\langle k\rangle,
$ which is independent of $k_{i}$. However, as
mentioned above, real networks often display degree-degree correlations, with the result
that $k_{nn,i}=k_{nn}(k_{i})$. If $k_{nn}(k)$ increases (decreases)
with $k$, the network is assortative (disassortative). A measure of
this phenomenon is Pearson's coefficient applied to the
edges \cite{Newman_rev, Newman_mixing_PRL, Newman_mixing_PRE, Boccaletti}: $ r= ([
k_{l}k'_{l}]-[ k_{l}]^{2})/([ k_{l}^{2}]-[ k_{l}]^{2}), $ where
$k_{l}$ and $k'_{l}$ are the degrees of each of the two nodes
belonging to edge $l$, and $[\cdot]\equiv(\langle k\rangle
N)^{-1}\sum_{l}(\cdot)$ is an average over edges. Writing
$\sum_{l}(\cdot)=\sum_{ij}\hat{a}_{ij}(\cdot)$, $r$ can be expressed
as
\begin{equation}
  r=\frac{\langle k\rangle \langle k^{2} k_{nn}(k)\rangle - 
    \langle k^{2}\rangle^{2} }{\langle k\rangle \langle k^{3}\rangle 
    - \langle k^{2}\rangle^{2}}.
  \label{r_gen}
\end{equation}
\begin{figure}
[tbh]
\begin{center}
\includegraphics
%[height=4.4cm,width=8.6cm]%
%[height=7.7cm,width=15.025cm]
[height=7.9cm,width=15.025cm]
%[scale=0.75]
{PRL/fig2_PRL.eps}
\caption{(Color online) Shannon entropy of correlated scale-free networks
against parameter $\beta$ (left panel) and
  against Pearson's coefficient $r$ (right panel), for various
  values of $\gamma$ (increasing from bottom to top). $\langle
  k\rangle=10$, $N=10^{4}$.  }%
\label{fig_ent}%
\end{center}
\end{figure}
The ensemble of all networks with a given degree sequence $(k_{1},...k_{N})$
contains a subset for all members of which $k_{nn}(k)$ is constant (the configuration ensemble), but also subsets displaying other functions $k_{nn}(k)$. We can identify each one of these subsets (regions of phase space) with an
expected adjacency matrix $\hat{\epsilon}$ which simultaneously satisfies the following conditions: ${\bf i)}$  $\sum_{j}k_{j}\hat{\epsilon}_{ij}=k_{i}k_{nn}(k_{i})$, $\forall i$, and ${\bf ii)}$ $\sum_{j}\hat{\epsilon}_{ij}=k_{i}$, $\forall i$ (for consistency). An ansatz which fulfills these requirements is any matrix of the form
\begin{equation}
  \hat{\epsilon}_{ij}=\frac{k_{i}k_{j}}{\langle k\rangle N}
%  \nonumber
  +\int d\nu \frac{f(\nu)}{N}\left[\frac{(k_{i}k_{j})^{\nu}}
    {\langle k^{\nu}\rangle}-k_{i}^{\nu}-k_{j}^{\nu}+\langle k^{\nu}\rangle  \right],
\label{epsi_gen}
\end{equation}
where 
$\nu\in\mathbb{R}$ and the function $f(\nu)$
is in general arbitrary,
although depending on the degree sequence
it shall here be restricted to values
which maintain $\hat{\epsilon}_{ij}\in [0,1]$, $\forall i,j$. This ansatz yields
\begin{eqnarray}
  k_{nn}(k)=\frac{\langle k^{2}\rangle}{\langle k\rangle}
  +\int d\nu f(\nu)\sigma_{\nu+1}\left[\frac{k^{\nu-1}}
    {\langle k^{\nu}\rangle}-\frac{1}{k} \right]
\label{knn_gen}
\end{eqnarray}
(the first term being the result for the
configuration ensemble), where $\sigma_{b+1}\equiv \langle k^{b+1}\rangle -\langle k\rangle
\langle k^{b}\rangle$.
In practice, one could adjust Eq. (\ref{knn_gen}) to fit any
given function $k_{nn}(k)$ and then wire up a network with the desired correlations: it suffices to throw random numbers
according to Eq. (\ref{epsi_gen}) with
$f(\nu)$ as
obtained from
the fit to Eq. (\ref{knn_gen})\footnote{Although, as with the configuration ensemble,
  it is not always possible to wire a network according to a
  given $\hat{\epsilon}$.}. To prove the uniqueness of a matrix $\hat{\epsilon}$ obtained in this way (i.e., that it is the only one compatible with a given $k_{nn}(k)$) assume that there exists another valid matrix $\hat{\epsilon}'\neq\hat{\epsilon}$. Writting $\hat{\epsilon}_{ij}'-\hat{\epsilon}_{ij}\equiv h(k_{i},k_{j})=h_{ij}$, then ${\bf i)}$ implies that $\sum_{j}k_{j}h_{ij}=0$, $\forall i$, while ${\bf ii)}$ means that $\sum_{j}h_{ij}=0$, $\forall i$. It follows that $h_{ij}=0$, $\forall j$.
\\
\linebreak

In many empirical networks, $k_{nn}(k)$ has the form $k_{nn}(k)=A+B
k^{\beta}$, with $A,B>0$ \cite{Boccaletti, Pastor-Satorras} -- the
mixing being assortative (disassortative) if $\beta$ is positive
(negative). Such a case is fitted by Eq. (\ref{knn_gen}) if $f(\nu)=C[\delta(\nu-\beta-1)\sigma_{2}/\sigma_{\beta+2}-\delta(\nu-1)]$, with $C$ a positive constant, since this choice yields
\begin{equation}
  k_{nn}(k)=\frac{\langle k^{2}\rangle}{\langle k\rangle}
  +C\sigma_{2}\left[\frac{k^{\beta}}{\langle
      k^{\beta+1}\rangle}-\frac{1}{\langle k\rangle} \right].
\label{knn_simple}
\end{equation}
After plugging Eq. (\ref{knn_simple}) into Eq. (\ref{r_gen}), one obtains:
\begin{equation}
  r=\frac{C\sigma_{2}}{\langle k^{\beta+1}\rangle}
  \left(\frac{\langle k\rangle \langle k^{\beta+2} \rangle - 
      \langle k^{2}\rangle\langle k^{\beta+1}\rangle }
{\langle k\rangle \langle k^{3}\rangle - \langle k^{2}\rangle^{2}}\right).
\label{r_simple}
\end{equation}
Inserting Eq. (\ref{epsi_gen}) in Eq. (\ref{eq_s_exact}), we can calculate the
entropy of 
correlated
networks
as a function of $\beta$ and $C$ -- or,
by using Eq. (\ref{r_simple}),
as a function of $r$. Particularizing for scale-free networks, then given
$\langle k\rangle$, $N$ and $\gamma$, there is always a certain combination of
parameters $\beta$ and $C$ which maximizes the entropy; we shall call these
$\beta^{*}$ and $C^{*}$.  For $\gamma\lesssim 5/2$ this point corresponds
to $C^{*}=1$. For higher $\gamma$, the entropy can be slightly higher for
larger $C$.
However, for these
values of $\gamma$, the assortativity $r$ of the point of maximum entropy
obtained with $C=1$ differs very little from the one corresponding to
$\beta^{*}$ and $C^{*}$ (data not shown). Therefore, for the sake of
clarity but with very little loss of accuracy, in the following we shall
generically set $C=1$ and vary only $\beta$ in our search for the level
of assortativity, $r^{*}$, that maximizes the entropy given $\langle
k\rangle$, $N$ and $\gamma$.  Note that $C=1$ corresponds to removing the
linear term, proportional to $k_i k_j$, in Eq. (\ref{epsi_gen}), and leaving
the leading non-linearity, $(k_i k_j)^{\beta+1}$, as the dominant one.
\begin{figure}
[tbh]
\begin{center}
\includegraphics
%[height=5.5cm,width=7.5cm]%
[scale=0.75]
{PRL/fig3_PRL.eps}
\caption{(Color online)
Lines from top to bottom: $r$ at which the entropy is maximized, $r^{*}$, against $\gamma$ for random scale-free networks with mean degrees $\langle k\rangle=\frac{1}{2}$, $1$, $2$ and $4$ times $k_{0}=5.981$, and $N=N_{0}=10697$ nodes ($k_{0}$ and $N_{0}$ correspond to the values for the Internet at the AS level in $2001$ \cite{Park_correlations}, which had $r=r_{0}=-0.189$). Symbols are the values obtained in \cite{Park_correlations} as those expected solely due to the one-edge-per-pair restriction (with $k_{0}$, $N_{0}$ and $\gamma=2.1$, $2.3$ and $2.5$). Inset: $r^{*}$ against $N$ for networks with fixed $\langle k\rangle/N$ (same values as the main panel) and $\gamma=2.5$; the arrow indicates $N=N_{0}$.
}%
\label{fig_max}%
\end{center}
\end{figure}

Fig. \ref{fig_ent} displays the entropy curves for various scale-free
networks, both as functions of $\beta$ and of $r$: {\it depending on
  the value of $\gamma$, the point of maximum entropy can be either
  assortative or disassortative}. This can be seen more clearly in
Fig. \ref{fig_max}, where $r^{*}$ is plotted against $\gamma$ for
scale-free networks with various mean degrees $\langle k\rangle$.
% Bit about the Pauli effect:
The values obtained by Park and Newman \cite{Park_correlations} as those resulting from the one-edge-per-pair restriction are also shown for comparison: notice that whereas this effect alone cannot account for the Internet's correlations for any $\gamma$, entropy considerations would suffice if $\gamma\simeq2.1$.
As shown in the inset, the results are robust in the large system-size limit.

Since most networks observed in the real world are highly
heterogeneous, with exponents in the range $\gamma\in (2,3)$, it is to
be expected that these should display a certain disassortativity --
the more so the lower $\gamma$ and the higher $\langle k\rangle$. In
Fig. \ref{fig_all} we test this prediction on a sample of empirical,
scale-free networks quoted in Newman's review \cite{Newman_rev} (p. 182). For each case, we found the value of $r$ that maximizes $S$
according to Eq. (\ref{eq_s_exact}), after inserting
Eq. (\ref{epsi_gen}) with the quoted values of $\langle k\rangle$, $N$
and $\gamma$.
In this way, we obtained the expected
assortativity for six networks, representing: a peer-to-peer (P2P)
network, metabolic reactions, the nd.edu domain, actor collaborations,
protein interactions, and the Internet (see \cite{Newman_rev} and
references therein).  For the metabolic, Web domain and protein
networks, {\it the values predicted are in excellent agreement with
  the measured ones}; therefore, no specific anticorrelating mechanisms need to
be invoked to account for their disassortativity. In the other three
cases, however, the predictions are not accurate, so there must be
additional
correlating mechanisms at work. Indeed, it is known that small
routers tend to connect to large ones \cite{Pastor-Satorras}, so one
would expect the Internet to be more disassortative than predicted, as
is the case\footnote{However, as Fig. \ref{fig_max} shows, if the Internet exponent were the $\gamma=2.2\pm0.1$ reported in \cite{Pastor-Satorras} rather than $\gamma=2.5$, entropy would account more fully for these correlations.} -- an effect that is less pronounced but still detectable
in the more egalitarian P2P network. Finally, as is typical of social
networks, the actor graph is significantly more assortative than
predicted, probably due to the homophily mechanism whereby highly
connected, big-name actors tend to work together \cite{Newman_mixing_PRL, Newman_mixing_PRE}.
\begin{figure}
[tbh]
\begin{center}
\includegraphics
%[height=5.5cm,width=7.5cm]%
[scale=0.75]
{PRL/fig4_PRL.eps}
\caption{(Color online) Level of assortativity that maximizes the
  entropy, $r^{*}$, for various real-world, scale-free networks, as
  predicted theoretically by Eq. (\ref{eq_s_exact}) (solid symbols)
  and as directly measured (empty symbols), against exponent $\gamma$.
}%
\label{fig_all}%
\end{center}
\end{figure}

\section{To sum up...}

In summary, we have shown how
the ensemble of networks with a given degree sequence can be partitioned
into regions of equally correlated networks and found, using an information-theory approach, that
the largest (maximum entropy) region, for the case of scale-free networks, usually displays a certain disassortativity. Therefore, in the absence of knowledge regarding the specific evolutionary forces at work, this should be considered the most likely state.
Given the accuracy with which our approach can predict
the degree of assortativity of certain empirical networks {\it with no
  a priori information thereon}, we suggest this as a neutral model to
decide whether or not particular experimental data require specific
mechanisms to account for observed degree-degree
correlations.

\section*{Acknowledgements}

This work was supported by the Junta de Andaluc\'{i}a project
P09-FQM4682, and by Spanish MICINN--FEDER project FIS2009--08451.





==> pub/pub_old.tex <==
%\documentclass[a4paper,10pt]{article}
%\usepackage{graphicx}
%\usepackage{amssymb}

\chapter{Selected publications} % Write in your own chapter title
\label{Appendix_PUB}
\lhead{\emph{Selected publications}} % Write in your own chapter title to set the page header


%\begin{center}
%\author{\bf S. Johnson, J. Marro, and J.J. Torres}
%\end{center}


\begin{itemize}
 \item 
Cluster Reverberation: a mechanism for robust short-term memory without synaptic learning, S. Johnson, J. Marro,  and JJ. Torres,  submitted, arXiv:1007.3122
\item
Enhancing neural-network performance via assortativity, S. de Franciscis, S. Johnson, and J.J. Torres, Phys. Rev E, in press. arXiv:1012.1813
\item
Nonequilibrium behavior in neural networks: criticality and optimal performance, J.J. Torres, S. Johnson, J.F. Mejias, S. de Franciscis and J. Marro, Lecture Notes in Computer Science, in press.
\item
Entropic origin of disassortativity in complex networks, S. Johnson, J.J. Torres, J. Marro, and M.A. Muñoz, Physical Review Letters 104, 108702 (2010)
\item
Evolving networks and the development of neural systems, S. Johnson, J. Marro and J.J. Torres, Journal of Statistical Mechanics (2010) P03003
\item
Excitable networks: nonequilibrium criticality and optimum topology, J.J. Torres, S. de Franciscis, S. Johnson, and J. Marro, International Journal of Bifurcation and Chaos 20, 869-875 (2010)
\item
Development of neural network structure with biological mechanisms, S. Johnson, J. Marro, J.F. Mejias, and J.J. Torres, Lecture Notes in Computer Science 5517, 228-235 (2009)
\item
Switching dynamics of neural systems in the presence of multiplicative colored noise, J.F. Mejias, J.J. Torres, S. Johnson, and H.J. Kappen, Lecture Notes in Computer Science 5517, 17-23 (2009)
\item
Nonlinear preferential rewiring in fixed-size networks as a diffusion process, S. Johnson, J. J. Torres, and  J. Marro, Physical Review E 79, 050104(R) (2009)
\item
Functional optimization in complex excitable networks, S. Johnson., J. Marro, and J.J. Torres, EPL 83, 46006(1-6) (2008)

\end{itemize}



==> rap/rap_old.tex <==
\chapter{Nonlinear preferential rewiring in fixed-size networks as a diffusion process} % Write in your own chapter title
\label{Appendix_RAP}
\lhead{Appendix A \emph{Nonlinear preferential rewiring in fixed-size networks as a diffusion process}} % Write in your own chapter title to set the page header

\begin{center}
\author{\bf S. Johnson, J. Marro, and J.J. Torres}
\end{center}

%\begin{abstract}
\begin{quotation}
\begin{center}
{\bf Abstract}
\end{center}
We present an evolving network model in which the total numbers of nodes and
edges are conserved, but in which edges are continuously rewired according to
nonlinear preferential detachment and reattachment. Assuming power-law kernels
with exponents $\alpha$ and $\beta$, the stationary states the degree
distributions evolve towards exhibit a second order phase transition -- from
relatively homogeneous to highly heterogeneous (with the emergence of starlike
structures) at $\alpha=\beta$. Temporal evolution of the distribution in this
critical regime is shown to follow a nonlinear diffusion equation, arriving at
either pure or mixed power-laws, of exponents $-\alpha$ and $1-\alpha$.
\end{quotation}




%\pacs{05.40.-a, 05.10.-a, 89.75.-k, 64.60.aq}

% 05.40.-a 	Fluctuation phenomena, random processes, noise, and Brownian motion
% 05.10.-a 	Computational methods in statistical physics and nonlinear dynamics
% 89.75.-k 	Complex systems
% 64.60.aq 	Networks

%\maketitle


Complex systems may often be described as a set of nodes with edges connecting some of them
-- the \textit{neighbours --} (see, for instance, Refs.\cite{Boccaletti,Arenas_rev,Marro_complex}).
The number of edges a particular node has is called its degree, $k$. The study of such large 
networks is usually made simpler by considering statistical properties, e.g.,
the degree distribution, $p(k)$ (probability of finding a node with a
particular degree). It turns out that a high proportion of real-world networks
follow power-law degree distributions, $p(k)\sim k^{-\gamma}$ -- referred to
as \textit{scale-free} due to their lack of a characteristic size. Also, many
of them have their edges placed among the nodes apparently in a random way
-- i.e., there is no correlation between the degree of a node and any other of
its properties, such as the degrees of its neighbours. Barab\'{a}si and Albert \cite{Barabasi} applied the mechanism of \textit{preferential attachment} to an evolving network model and showed how this resulted in the degree distributions becoming scale-free for long enough times. For this to work, attachment had to be linear -- i.e., the probability a node with degree $k$ has of receiving a new edge is $\pi(k)\sim k+q$. This results in scale-free stationary degree distributions with an exponent $\gamma=3-q$.

Preferential attachment seems to be behind the emergence of many real-world,
continuously growing networks. However, not all networks in which some nodes at times gain (or loose) new edges have a continuously growing number of nodes. For example, a given group
of people may form an evolving social network \cite{Kossinets} in which the
edges represent friendship. Preferential attachment may be relevant here -- the more people you know, the more likely it is that you will be introduced
to someone new -- but probabilities are not expected to depend linearly on
degree. For instance, there may be saturations (highly connected people might
become less accessible), threshold effects (hermits may be prone to antisocial
tendencies), and other non-linearities. The brain may also be a relevant case.
Once formed, the number of neurons does not seem to continually augment, and
yet its structural topology is dynamic \cite{Klintsova}. Synaptic growth and
dendritic arborization have been shown to increase with electric stimulation
\cite{Lee,DeRoo} -- and, in general, the more connected a neuron is, the more
current it receives from the sum of its neighbours.

Barab\'{a}si and Albert showed that both (linear) preferential attachment and
an ever-growing number of nodes are needed for scaling to emerge in their
model. In a fixed population, their mechanism would result in a
fully-connected network. However, this is not normally observed in real
systems. Rather, just as some new edges sprout, others disappear -- less used
synapses suffer atrophy, unstimulating friendships wither. Often, the numbers
of both nodes and edges remain roughly constant. The same authors did
therefore extend their model so as to include the effects of
\textit{preferential rewiring} (which could be applied to fixed-size
networks), although again probabilities depended linearly on node degree
\cite{Albert}. Another mechanism which (roughly) maintains constant the
numbers of nodes and edges is node fusing \cite{Thurner}, once more according
to linear probabilities. As to nonlinear preferential attachment, the
(growing) BA model was extended to take power-law probabilities into account
\cite{Krapivsky}, although the solutions are only scale free for the linear case.

In this note we present an evolving network model with preferential rewiring
according to nonlinear (power-law) probabilities. The number of nodes and
edges is conserved but the topology evolves, arriving eventually at a
macroscopically (nonequilibrium) stationary state -- as described by global
properties such as the degree distribution. Depending on the exponents chosen
for the rewiring probabilities, the final state can be either fairly
homogeneous, with a typical size, or highly heterogeneous, with the emergence
of starlike structures. In the critical case marking the transition between
these two regimes, the degree distribution is shown to follow a nonlinear
diffusion equation. This describes a tendency towards stationary states that are
characterized either by scale-free or by mixed scale-free distributions,
depending on parameters.

Our model consists of a random network with $N$ nodes of respective degree
$k_{i},$ $i=1,2,...,N,$ and $%
\frac12 N\left\langle k\right\rangle $ edges. Initially, the degrees have a given
distribution $p(k,t=0)$. At each time step, one node is chosen with a
probability which is a function of its degree, $\rho(k_{i})$. One of its edges
is then chosen randomly and removed from it, to be reconnected to another node
$j$ chosen according to a probability $\pi(k_{j})$. That is, an edge is broken
and another one is created, and the total number of edges, as well as the
total number of nodes, is conserved. The functions $\pi(k)$ and $\rho(k)$ are
arbitrary, but we shall explicitly illustrate here $\pi(k_{i})\sim
k_{i}^{\alpha}$ and $\rho(k_{i})\sim k_{i}^{\beta}$ that capture the essence
of a wide class of nonlinear monotonous response functions and are easy to
handle analytically.

The probabilities $\pi$ and $\rho$ a given node has, at each time step, of
increasing or decreasing its degree can be interpreted as transition
probabilities between states. The expected value of the increment in a given
$p(k,t)$ at each time step, $\Delta p(k,t)$, may then be written as%

\begin{align}
\frac{\partial p(k,t)}{\partial t}  &  =(k-1)^{\alpha}\,\bar{k}_{\alpha}%
^{-1}p(k-1,t)\nonumber\\
&  +(k+1)^{\beta}\,\bar{k}_{\beta}^{-1}\,p(k+1,t)\label{master}\\
&  -\left(  k^{\alpha}\,\bar{k}_{\alpha}^{-1}+k^{\beta}\,\bar{k}_{\beta}%
^{-1}\right)  \,p(k,t),\nonumber
\end{align}
where $\bar{k}_{a}=\bar{k}_{a}\left(  t\right)  =\sum_{k}k^{a}p(k,t).$
If it exists, any stationary solution must satisfy the condition
$p_{\text{st}}(k+1)\,(k+1)^{\beta}\,\bar{k}_{\alpha}^{\text{st}}=p_{\text{st}%
}(k)\,k^{\alpha}\,\bar{k}_{\beta}^{\text{st}}$ which, for $k\gg 1$, implies
that
\begin{equation}
\frac{\partial p_{\text{st}}(k)}{\partial k}=\left(  \frac{\bar{k}_{\alpha
}^{\text{st}}}{\bar{k}_{\beta}^{\text{st}}}\frac{k^{\alpha}}{(k+1)^{\beta}%
}-1\right)  p_{\text{st}}(k). \label{det_bal}%
\end{equation}
Therefore, the distribution will have an extremum at 
$k_{e}=\left(  \bar
{k}_{\beta}^{\text{st}}/\bar{k}_{\alpha}^{\text{st}}\right)  ^{\frac{1}%
{\alpha-\beta}}$ (where we have approximated $k_{e}\simeq k_{e}+1$). If
$\alpha<\beta$, this will be a maximum, signalling the peak of the
distribution. On the other hand, if $\alpha>\beta$, $k_{e}$ will correspond to
a minimum. Therefore, most of the distribution will be broken in two parts,
one for $k<k_{e}$ and another for $k>k_{e}$. The critical case for
$\alpha=\beta$ will correspond to a monotonously decreasing stationary
distribution, but such that $\mbox{lim}_{k\rightarrow\infty}\partial
p_{st}(k)/\partial k=0$. In fact, Eq. (\ref{master}) is for this situation
($\alpha=\beta$) the discretised version of a nonlinear diffusion equation,
\begin{equation}
\frac{\partial p(k,\tau)}{\partial\tau}=\frac{\partial^{2}}{\partial k^{2}%
}[k^{\alpha}p(k,\tau)], \label{diff}%
\end{equation}
after dynamically modifying the time scale according to $\tau=t/\bar
{k}_{\alpha}\left(  t\right)  $. Ignoring, for the moment, border effects, the
solutions of this equation are of the form
\begin{equation}
p_{\text{st}}(k)\sim Ak^{-\alpha}+Bk^{-\alpha+1}, \label{sol}%
\end{equation}
with $A$ and $B$ constants. If $\alpha>2$, then given $A$ we can always find a
$B$ which allows $p_{\text{st}}(k)$ to be normalized in the thermodynamic
limit \footnote{Although all moments of $k$ will diverge unless $B=0$.}. For example, if the lower limit is $k\geq1$, then
$B=(\alpha-2)\left[  1-A/(\alpha-1)\right]  $. However, if $1<\alpha\leq2$,
then only $A$ can remain non-zero, and $p_{\text{st}}(k)$ will be a pure power
law. For $\alpha\leq1$, both constants must tend to zero as $N\rightarrow
\infty$.%
\begin{figure}
[tbh]
\begin{center}
\includegraphics
%[width=7.95cm]
[width=12.cm]
{RAP/fig1_RAP.eps}
\caption{(Color online) Degree distribution $p(k,t)$ at four different stages of evolution:
$t=10^{2}$ [(yellow) squares], $10^{3}$ [(blue) circles], $10^{4}$ [(red) triangles)] and $10^{5}$ MCS [(black) diamonds]. From top to bottom panels, subcritical ($\alpha=0.5$), critical ($\alpha=1$) and supercritical ($\alpha=1.5$) rewiring exponents. Symbols from MC simulations
and corresponding solid lines from numerical integration of Eq. (\ref{master}). $\beta=1$, $\langle k\rangle=10$ and $N=1000$ in all cases.}%
\label{fig1}%
\end{center}
\end{figure}
In finite networks, no node can have a degree larger than $N-1$ or lower than
$0$. In fact, one would usually wish to impose a minimum nonzero degree, e.g.
$k\geq1$. The temporal evolution of the degree distribution is illustrated in
Fig. \ref{fig1}. This shows the result of integrating Eq. (\ref{master}) for
$k\geq1,$ different times, $\beta=1,$ and three different values of $\alpha$,
along with the respective values obtained from Monte Carlo simulations.%

\begin{figure}
[tbh]
\begin{center}
\includegraphics
%[width=9.cm]%
[width=13.cm]
{RAP/fig2_RAP.eps}
\caption{(Color online) Adjusted variance $\sigma^{2}/\langle k\rangle^{2}$ of the degree
distribution after $2\times10^{5}$ MCS against $\alpha$, as obtained from
MC simulations, for system sizes $N=800$ [(yellow) squares], $1200$ [(blue) circles], $1600$ [(red) triangles] and $2000$ [(black) diamonds]. Top left inset shows final degree distributions for $\alpha=0.5$ [light gray (blue)], $1$ [dark gray (red)] and $1.5$ (black), with $N=1000$. Bottom right inset shows typical time series of $\sigma^{2}/\langle k\rangle^{2}$ for the same three values of $\alpha$ and $N=1200$. In all cases, $\beta=1$ and $\langle k\rangle=10$.}%
\label{fig2}%
\end{center}
\end{figure}

The main result may be summarized as follows. For $\alpha<\beta$, the network
will evolve to have a characteristic size, centred around $\langle k\rangle$.
At the critical case $\alpha=\beta$, all sizes appear, according either to a
pure or a composite power law, as detailed above.

If we impose, say, $k\geq1$, then starlike structures will emerge, with a great many nodes connected to just a few
hubs \footnote{There is a finite-size effect not taken into account by the theory -- but relevant when $\alpha>\beta$ -- which provides a natural lower cutoff for $p_{st}(k)$: if there are, say, $m$ nodes which are connected to the whole network, then the minimum degree a node can have is $m$.}.

Figure \ref{fig2} illustrates the second order phase transition undergone by
the variance of the final (stationary) degree distribution, depending on the
exponent $\alpha$, where $\beta$ is set to unity. It should be mentioned that
this particular case, $\beta=1$, corresponds to edges being chosen at random
for disconnection, since the probability of a random edge belonging to node
$i$ is proportional to $k_{i}$.

This topological phase transition is similar to the ones that have been described in equilibrium network ensembles defined via an energy function, in the so-called \textit{synchronic} approach to network analysis \cite{Farkas,Park_equilibrium,Burda,Derenyi}. However, our (nonequilibrium) model does not come within the scope of this body of work, since the rewiring rates cannot, in general, be derived from a potential. Furthermore, we are here concerned with the time evolution rather than the stationary states, making our approach \textit{diachronic.} 

Summing up, in spite of its simplicity, our model captures the essence of many
real-world networks which evolve while leaving the total numbers of nodes and
edges roughly constant. The grade of heterogeneity of the stationary
distribution obtained is seen to depend crucially on the relation between the
exponents modelling the probabilities a node has of obtaining or loosing a new
edge. It is worth mentioning that the heterogeneity of the degree distribution
of a random network has been found to determine many relevant behaviours and
magnitudes such as its clustering coefficient and mean minimum path
\cite{Newman_rev}, critical values related to the dynamics of excitable
networks \cite{Johnson}, or the synchronisability for systems of coupled
oscillators (since this depends on the spectral gap of the Laplacian matrix)
\cite{Barahona}.

The above shows how scale-free distributions, with a range of
exponents, may emerge for nonlinear rewiring, although only in the critical
situation in which the probabilities of gaining or loosing edges are the same.
We believe that this non-trivial relation between the microscopic rewiring
actions (governed in our case by parameters $\alpha$ and $\beta$) and the emergent
macroscopic degree distributions could shed light on a class of biological,
social and communications networks.

\section*{Aknowledgements}

This work was supported by Junta de Anadaluc\'{i}a project FQM-01505 and by Spanish MEC-FEDER
project FIS2009-08451
%FIS2005-00791.




==> resu/notes.tex <==
\chapter{Notes}
\label{Appendix_Notes}
\lhead{\emph{Notes}}


Physics is like sex: sure, it may give some practical results, but that's not why we do it." 
- 
  --  Richard P. Feynman 

“Research is formalized curiosity. It is poking and prying with a purpose.”

 Zora Neale Hurston quotes (American folklorist and Writer, 1903-1960)


“Research is what I'm doing when I don't know what I'm doing.”

 Werner von Braun quotes

I believe there is no philosophical high-road in science, with epistemological signposts. No, we are in a jungle and find our way by trial and error, building our road behind us as we proceed.

Max Born (1882-1970) German Physicist. Nobel Prize, 1954.

---


To say that a man is made up of certain chemical elements is a satisfactory description only for those who intend to use him as a fertilizer.
    Hermann Joseph Muller (1890-1967) U. S. geneticist. Nobel prize for medicine 1946.



One had to be a Newton to notice that the moon is falling, when everyone sees that it doesn't fall.
    Paul Valéry (1871-1945) French poet and philosopher.


